Re-evaluating Group Robustness via Adaptive Class-Specific Scaling

Group distributionally robust optimization, which aims to improve robust accuracies -- worst-group and unbiased accuracies -- is a prominent algorithm used to mitigate spurious correlations and address dataset bias. Although existing approaches have reported improvements in robust accuracies, these gains often come at the cost of average accuracy due to inherent trade-offs. To control this trade-off flexibly and efficiently, we propose a simple class-specific scaling strategy, directly applicable to existing debiasing algorithms with no additional training. We further develop an instance-wise adaptive scaling technique to alleviate this trade-off, even leading to improvements in both robust and average accuracies. Our approach reveals that a na\"ive ERM baseline matches or even outperforms the recent debiasing methods by simply adopting the class-specific scaling technique. Additionally, we introduce a novel unified metric that quantifies the trade-off between the two accuracies as a scalar value, allowing for a comprehensive evaluation of existing algorithms. By tackling the inherent trade-off and offering a performance landscape, our approach provides valuable insights into robust techniques beyond just robust accuracy. We validate the effectiveness of our framework through experiments across datasets in computer vision and natural language processing domains.

==> sections/measure.tex <==
 % !TEX root = ../main.tex
 
 
 \subsection{Robust Coverage for Measuring Group Robustness}
 \label{sec:robust_coverage}
 
 In the previous subsection, we have seen that there exists a clear trade-off between robust and average accuracies, and robust scaling can identify the optimal point for the target metric.
 However, it still reflects only a single point of the trade-off curve while ignoring all other possible Pareto optimums.
 For a more comprehensive view, we propose a convenient measurement to have a scalar summary of the robust-average accuracy curve.
%  However, there may still have some artifacts that 
%  For more reliable measurement, we propose the \textit{Robust Coverage} that considers the trade-off. 
 Formally, we define the \textit{Robust Coverage} as
 \begin{align}
     \text{Coverage} :=  \int_{c=0}^1\max_\mathbf{s}\big\{\text{UA}^\mathbf{s}|\text{AA}^\mathbf{s}\geq c\big\}dc 
     \approx  \sum_{d=0}^{D-1}\frac{1}{D}\max_\mathbf{s}\big\{\text{UA}^\mathbf{s}|\text{AA}^\mathbf{s}\geq \frac{d}{D}\big\}
     \label{eq:coverage}
 \end{align}
 where $\text{UA}^\mathbf{s}$ and $\text{AA}^\mathbf{s}$ denote the unbiased and average accuracies of applying (\ref{eq:rs}) with the scaling factor $\mathbf{s}$.
 $D = 1000$ is the number of slices for discretization.
 The robust coverage measures the area under the extended robust-average accuracy curve, where the maximum operation in~(\ref{eq:coverage}) finds the Pareto optimum for each threshold.
 We can adopt either UA or WA as a target metric of the robust coverage, referred to as unbiased or worst-group coverages, respectively, as visualized in Fig.~\ref{fig:worst_curve_all_pareto_celeba} and~\ref{fig:unbias_curve_all_pareto_celeba}, respectively.
%Fig.~\ref{fig:worst_curve_all_pareto_celeba} and~\ref{fig:unbias_curve_all_pareto_celeba} visualizes both robust coverage curves on the CelebA dataset, where UA and WA are adopted as a target metric, respectively.
%  $\text{UA}^\mathbf{s}$ can be replaced by worst-group accuracy, $\text{WA}^\mathbf{s}$.
 Please refer to our supplementary document for more discussions.
%  The robust coverage is useful in the model selection process, where we can select the model which has the highest robust coverage in the validation split.

 \iffalse
 \subsubsection{Robust coverage in test split}
 Robust coverage can be directly calculated in the validation split, but unfortunately, it is not available in the test split.
This is because we need to know the values of $\text{UA}^{\mathbf{s}}$ in advance to conduct max operation in \eqref{eq:coverage}, but we cannot use the information in the test set.
To bypass this issue, we first define the set of optimal scaling factors for each threshold in the validation split $\mathcal{S}_\text{val}$ as
  \begin{equation}
%      \mathcal{S}_\text{val} := \Big\{ \max_\mathbf{s}\big\{\text{UA}^\mathbf{s}|\text{AA}^\mathbf{s}\geq c\big\}~~\forall c \in [0, 1]
%      \Big\},
      \mathcal{S}_\text{val} := \Big\{ \max_\mathbf{s}\big\{\text{UA}_{\text{val}}^\mathbf{s}|\text{AA}_{\text{val}}^\mathbf{s}\geq \frac{d}{D} \big\}~~\text{for}~0 \leq d \leq D-1
      \Big\},
  \end{equation}
then the unbiased coverage of test split is calculated by
\begin{equation}
      \text{Test coverage} := \frac{1}{|\mathcal{S}_\text{val}|} \sum_\mathbf{s \in \mathcal{S}_\text{val}} \text{UA}_{\text{test}}^\mathbf{s}.
  \end{equation}
\fi
 
 
 \iffalse
 \begin{table}[t]
\begin{center}
\caption{The results of robust coverage on the CelebA dataset with the average of three runs (standard deviations in parenthesis).
%Unbiased and worst denote unbiased and worst-group accuracy, respectively.
}
\vspace{0.2cm}
\label{tab:celebA_coverage}
 \scalebox{0.85}{
\setlength\tabcolsep{4pt} 
\begin{tabular}{cl|cc|c}
\toprule
Dataset & Method & Worst-. Cov. & Unbiased Cov. & Worst-group Acc.  \\
\hline
%CelebA & ERM & 31.1(1.7) & 76.4(1.2) & {95.5(0.4)} \\
%CelebA & CR & 70.6(6.0) & 88.7(1.2) & {94.2(0.7)} \\
%CelebA & LfF~\citep{LfF} & 55.6(6.6) & 81.5(2.8) & {92.4(0.8)} \\
%CelebA & JTT~\citep{JTT}  &76.1(3.4) &85.9(0.3) &{89.5(1.2)} \\
%CelebA & Group DRO~\citep{GroupDRO} & 88.4(2.3) & 92.0(0.4) & {93.2(0.8)} \\
%CelebA & GR & 87.9(1.7) & 91.9(0.3) & {93.0(0.9)}\\
CelebA & ERM & 83.0(0.7) & 88.1(0.5) & 31.1(1.7) \\ % & 76.4(1.2) & {95.5(0.4)} \\
CelebA & CR & 82.9(0.5) & 88.2(0.3) & 70.6(6.0) \\ %& 88.7(1.2) & {94.2(0.7)} \\
CelebA & LfF~\citep{LfF} & 73.1(2.2) & 79.5(1.8) & 55.6(6.6) \\%& 81.5(2.8) & {92.4(0.8)} \\
CelebA & JTT~\citep{JTT}  &77.3(0.7) & 81.9(0.7) &76.1(3.4) \\% &85.9(0.3) &{89.5(1.2)} \\
CelebA & Group DRO~\citep{GroupDRO} &87.3(0.2) & 88.4(0.2)  & 88.4(2.3) \\% & 92.0(0.4) & {93.2(0.8)} \\
CelebA & GR &86.9(0.4) & 88.3(0.2) & 87.9(1.7) \\% & 91.9(0.3) & {93.0(0.9)}\\
\bottomrule
\end{tabular}
 }
\end{center}
%  \vspace{-0.1cm}
\end{table}
\fi

% \begin{table}[t]
%\begin{center}
%\caption{The results of robust coverage on the CelebA dataset with the average of three runs (standard deviations in parenthesis).
%%Unbiased and worst denote unbiased and worst-group accuracy, respectively.
%}
%\vspace{0.2cm}
%\label{tab:celebA_coverage}
% \scalebox{0.85}{
%\setlength\tabcolsep{4pt} 
%\begin{tabular}{cl|cc|c}
%\toprule
%Dataset & Method & Worst-group Cover. & Unbiased Cover. & Worst-group Acc.  \\
%\hline
%CelebA & ERM & 83.0(0.7) & 88.1(0.5) & 31.1(1.7) \\ % & 76.4(1.2) & {95.5(0.4)} \\
%CelebA & CR & 82.9(0.5) & 88.2(0.3) & 70.6(6.0) \\ %& 88.7(1.2) & {94.2(0.7)} \\
%CelebA & LfF~\citep{LfF} & 73.1(2.2) & 79.5(1.8) & 55.6(6.6) \\%& 81.5(2.8) & {92.4(0.8)} \\
%CelebA & JTT~\citep{JTT}  &77.3(0.7) & 81.9(0.7) &76.1(3.4) \\% &85.9(0.3) &{89.5(1.2)} \\
%CelebA & Group DRO~\citep{GroupDRO} &87.3(0.2) & 88.4(0.2)  & 88.4(2.3) \\% & 92.0(0.4) & {93.2(0.8)} \\
%CelebA & GR &86.9(0.4) & 88.3(0.2) & 87.9(1.7) \\% & 91.9(0.3) & {93.0(0.9)}\\
%\bottomrule
%\end{tabular}
% }
%\end{center}
%%  \vspace{-0.1cm}
%\end{table}
 
 
 % This is more reliable than using the robust accuracy of a single point.
 %% model selection 결과 필요.
 
 

 
  \iffalse
 We clarify that measuring the exact robust coverage in the test set is not possible, because it contains the maximum operation which requires the knowledge of test set results.
 Nevertheless, we use the robust coverage as an additional metric because it gives a tight upper bound.
 We also observe that the robust coverage of validation and test sets are almost the same.
%  As in Figure~\ref{}, we observe that the optimal points which gives the maximum UA given of the validation set is mostly aligned well to that of the test set. 
 Please refer to the supplementary document for more details about this issue.
 \fi
%  However, we observe that the optimal points of the validation set is mostly aligned well to that of the test set. ...
 
 
 % Figure needed.
 
%  \subsubsection{Results}
%  We evaluated robust coverage of existing approaches and ERM baseline.
 
 

==> sections/method.tex <==
 % !TEX root = ../main.tex
 

 
 
 
% \subsection{Group Robust Methods with Adaptive Robust Scaling}
% \subsection{Instance-wise Robust Scaling for Improving Group Robustness}
 \subsection{Instance-wise Robust Scaling}
 \label{sec:method}
The optimal scaling factor can be applied adaptively to each test example and the instance-specific scaling has the potential to overcome the trade-off and improve accuracy even further.  
Previous approaches~\cite{seo2021unsupervised, sohoni2020no} have shown the capability to identify hidden spurious attributes via clustering on the feature space for debiased representation learning.
Likewise, we take advantage of feature clustering for adaptive robust scaling; we obtain the optimal class-specific scaling factors based on the cluster membership for each sample.
The overall algorithm of instance-wise robust scaling (IRS) is described as follows.

\begin{enumerate}
  \item Perform clustering with validation data on the feature space and store the cluster centroids.   \item Find the optimal scaling factor for each cluster.
%  \item Assign each test example to the nearest cluster using the stored cluster centroids in step 1.\vspace{-0.05cm}
%  \textbf{4)} Apply the optimal scaling factors obtained in 2) to the samples of each cluster in the test split.
  \item Apply the estimated scaling factor to the test example based on its cluster membership.
\end{enumerate}

In step 1, we use a simple \textit{k}-means clustering algorithm, where the number of clusters $K$ is set to the value that gives the highest robust coverage in the validation set. 
Empirically, numbers larger than 10, \ie, $K > 10$, yield stable and superior results, compared to the original class-specific scaling.







==> sections/method_ars.tex <==
 % !TEX root = ../main.tex
 
 
% \subsection{Group Robust Methods with Adaptive Robust Scaling}
 \subsection{Group Robust Methods with Instance-wise Robust Scaling}
 \label{sec:method}
%This subsection provides two extended models based on the robust scaling strategy, each of which can be utilized with or without explicit knowledge of group information, respectively.
%If we partition the dataset based on feature semantics and reserve different scaling factors for each partition, then it can give more flexible trade-offs. 
For each test example, if we can apply instance-wise scaling factors based on its feature semantics, then it will improve the trade-off furthermore.  
This subsection provides two practical methods to implement it based on the robust scaling strategy, each of which can be utilized with or without  the supervision of group information during training, respectively.
 
 \iffalse
 \subsubsection{Attribute-Specific Robust Scaling (ARS)}
 \label{sec:ars}
% If we partition the dataset based on feature semantics and reserve different scaling factors for each partition, then it can give more flexible trade-offs. 
%From this intuition, we partition the examples based on the values of spurious attributes, and we call each partition as attribute-group.
%From this intuition, 
We first partition the examples based on the values of spurious attributes.
Like as the original robust scaling procedure, we obtain the optimal scaling factors for each partition in the validation split and apply them to the test split.
However, this partition-wise scaling is basically unavailable because we do not know the spurious attribute values of the examples in the test split, so we need to estimate those values.
%However, because we do not know the spurious attribute values of the examples in the test split, we need to estimate their values for partition-wise scaling. 
%To this end, we follow a simple algorithm described in Alg.~\ref{alg:ars}.
To this end, we follow a simple algorithm described below:

%\begin{enumerate}[label=\arabic*)]
%%  \item Using the ground-truth values of spurious attribute, find the optimal scaling factors for each bias-group in the validation split.
%  \item Partition the validation examples by the values of the spurious attribute.
%  \item Find the optimal scaling factors for each partition in the validation split.
%  \item Train an independent estimator model to classify spurious attribute.
%  \item Estimate the spurious attribute values of the examples in the test split using the model trained from 3).
%  \item Partition the test samples according to their estimated spurious attribute values, and apply the optimal scaling factors obtained in 2).
%\end{enumerate}
\textbf{1)} Partition the validation examples by the values of the spurious attribute.\\
\textbf{2)} Find the optimal scaling factors for each partition in the validation split. \\
\textbf{3)} Train an independent estimator model to classify spurious attribute. \\
\textbf{4)} Estimate the spurious attribute values of the examples in the test split using the estimator, and partition the test samples according to their estimated spurious attribute values. \\
\textbf{5)} Apply the optimal scaling factors obtained in 2) to the samples of each partition in the test split.

To find a set of scale factors corresponding to each partition, we adopt a na\"ive greedy algorithm that performed in one partition at a time.
This attribute-specific robust scaling further increases the robust accuracy compared to the original robust scaling, and also improves the robust coverage.
One limitation is that it requires the supervision of spurious attribute information to train the estimator model in 3). 
However, we notice that only a very few examples with the supervision is enough to train the spurious-attribute estimator, because it is much easier to learn as the word ``spurious correlation" suggests.
 
 \fi
%\begin{algorithm}[t]
%\small
%\SetAlgoLined
%\textbf{1)} Partition the validation examples by the values of the spurious attribute.\\
%\textbf{2)} Find the optimal scaling factors for each partition in the validation split. \\
%\textbf{3)} Train an independent estimator model to classify spurious attribute. \\
%\textbf{4)} Estimate the spurious attribute values of the examples in the test split using the estimator, and partition the test samples according to their estimated spurious attribute values. \\
%\textbf{5)} Apply the optimal scaling factors obtained in 2) to each partition in the test split.
%\caption{Attribute-specific Robust Scaling (ARS)}
%\label{alg:ars}
%\end{algorithm}
%
  % 
% \subsection{Cluster Robust Scaling (CRS)}
 \subsubsection{Cluster-Specific Robust Scaling (CRS)}
 \label{sec:crs}
%As we mentioned in the previous subsection, although the bias-group robust scaling works well, the requirement of explicit bias supervision limits the practicality of the method.
As we mentioned in the previous subsection, the requirement of explicit group supervision can limit the practicality of the method to some extent.
To overcome this limitation, we take advantage of feature clustering for partitioning in an unsupervised way.
Previous approaches~\citep{seo2021unsupervised, sohoni2020no} have showed the capability to identify hidden spurious attributes via clustering on the feature space.
%The overall algorithm is described in Alg.~\ref{alg:crs}.
The overall algorithm is described as follows.

  \textbf{1)} Clustering the examples on the feature space in the validation split and store the centroids of the clusters. \\
  \textbf{2)} Find the optimal scaling factors for each cluster in the validation split. \\
  \textbf{3)} Assign the examples in the test split to the clusters by selecting their nearest centroids obtained from 1). \\
  \textbf{4)} Apply the optimal scaling factors obtained in 2) to the samples of each cluster in the test split.

%\begin{enumerate}[label=\arabic*)]
%  \item Clustering the examples on the feature space in the validation split and store the centroids.
%  \item Find the optimal scaling factors for each cluster in the validation split.
%  \item Assign the examples in the test split to the clusters by selecting their nearest centroids from 1).
%  \item Apply the optimal scaling factors obtained in 2).
%\end{enumerate}
%\\
%\\
%1) Clustering the examples on the feature space in the validation split and store the centroids.\\
%2) Find the optimal scaling factors for each cluster in the validation split.\\
%3) Assign the examples in the test split to the clusters by using the centroids from 1).\\
%4) Apply the optimal scaling factors from 2).\\
%
In 1), we use the na\"ive \textit{k}-means algorithm for clustering.
The number of clusters $K$ is a hyperparameter to be chosen, but it can be easily tuned by selecting the best number that gives the highest robust coverage in the validation split. 
We found that a sufficient number of $K > 10$ gives stable and superior results, compared to the original robust scaling.


==> sections/prelim_supple.tex <==
 % !TEX root = ../main.tex
 
% 
% \section{Preliminaries}
% \label{sec:prelim}
%
% \subsection{Problem Setup}
% Let consider a triplet $(x, y, a)$ consisting of an input feature $x \in \mathcal{X}$, a target label $y \in \mathcal{Y}$, and a spurious attribute $a \in \mathcal{A}$. 
% We define the group as a pair of target label and spurious attribute, $g := (y, a) \in \mathcal{Y} \times \mathcal{A} =: \mathcal{G}$.
% We are basically given $n$ training examples without group annotations, \eg, $\{(x_1, y_1), ..., (x_n, y_n)\}$, while given $m$ validation examples with group annotations for model selection, \eg, $\{(x_1, g_1), ..., (x_m, g_m)\}$ = $\{(x_1, y_1, a_1), ..., (x_m, y_m, a_m)\}$.
% 
%% \begin{align}
%%     \text{UA} := \frac{1}{N}\sum_{i=1}^N \mathbf{1}(f_\theta(\mathbf{x}_i) = y_i )
%% \end{align}
% Our goal is to learn a model $f_\theta(\cdot): \mathcal{X} \rightarrow \mathcal{Y}$ that is robust to group distribution shifts.
%%  To evaluate the group robustness, let first define the group-wise accuracy (GA).
% To measure the group robustness, unbiased accuracy (UA) and worst-group accuracy (WA) are usually adopted.
% Let first define the group-wise accuracy (GA):
% \begin{align}
%    \text{GA}_{(r)} := \frac{\sum_{i} \mathds{1}(f_\theta(\mathbf{x}_i) = y_i, g_i=r)}{\sum_{i} \mathds{1}(g_i=r)},
%\end{align}
%where $\mathds{1}(\cdot)$ is an indicator function and $\text{GA}_{(r)}$ denotes the accuracy of $r^\text{th}$ group samples.
%Unbiased and worst-group accuracies are defined by
%\begin{align}
%    \text{UA} := \frac{1}{|\mathcal{G}|}\sum_{r\in\mathcal{G}}{\text{GA}_{(r)}},~~~~~ \text{WA} := \max_{r\in\mathcal{G}} \text{GA}_{(r)},
%\end{align}
%both of which are also referred to as robust accuracy.
% 
% \subsection{Comparisons} 
%%Below is a brief introduction of the comparisons used in our experiments.
%
% \paragraph{ERM}
% Given a loss function $\ell(\cdot)$, the objective of empirical risk minimization is optimizing the following loss over training data: 
% \begin{align}
%    %  \min_\theta \Big\{ \mathcal{L}_\text{ERM}(f_\theta) := \mathbb{E}_{(x,y,a)\sim P}[\ell(f_\theta(x), y)] \Big\}
%    \min_\theta \Big\{\frac{1}{n}\sum_{i=1}^n \ell(f_\theta(x_i), y_i) \Big\}.
% \end{align}
%%  where $P$ is the empirical distribution over training data.
% 
% \paragraph{Class reweighting (CR)}
% To mitigate the class imbalance issue, we can simply reweight the samples based on the inverse of class frequency in the training split, 
%  \begin{align}
%    \min_\theta \Big\{\frac{1}{n}\sum_{i=1}^n \omega_i \ell(f_\theta(x_i), y_i) \Big\}~~\text{where}~~\omega_i = \frac{n}{\sum_j \mathds{1}(y_j=y_i)}
% \end{align}
% 
% \paragraph{LfF}
%Motivated by the observation that bias-aligned samples are more easily learned, LfF~\citep{LfF} simultaneously trains a pair of neural network $(f_B, f_D)$.
%The biased model $f_B$ is trained with generalized cross-entropy loss which intends to amplify bias, while the debiased model $f_D$ is trained with a standard cross-entropy loss, where each sample $(x_i, y_i)$ is reweighted by the following relative difficulty score:
%\begin{align}
%%    \omega_i = \frac{\log f_B(y_i|x_i)}{\log f_B(y_i|x_i) + \log f_D(y_i|x_i)}.
%    \omega_i = \frac{\ell(f^B_\theta(x_i), y_i)}{\ell(f^B_\theta(x_i), y_i) + \ell(f^D_\theta(x_i), y_i)}.
%\end{align}
%
% 
%
% \paragraph{JTT}
% JTT~\citep{JTT} consists of two-stage procedures. In the first stage, JTT trains a standard ERM model $\hat{f}(\cdot)$ for several epochs and identifies an error set $E$ of training examples that are misclassified:
% \begin{align}
%E := \{(x_i, y_i)~~\text{s.t.}~\hat{f}(x_i) \neq y_i \}.
% \end{align}
% Next, they train a final model $f_\theta(\cdot)$ by upweighting the examples in the error set $E$ as
% \begin{align}
%      \min_\theta \Big\{  \lambda_\text{up}\sum_{(x,y)\in E}\ell(f_\theta(x), y) + \sum_{(x,y)\notin E}\ell(f_\theta(x), y) \Big\}.
% \end{align}
% 
% 
% 
% \paragraph{Group DRO}
%%  While ERM is the standard way and generally works well, it often learns spurious correlation and consequently, it leads to poor robust accuracy.
%%  To tackle this problem, Group DRO aims to minimize the worst-group loss formulated as:
%Group DRO~\citep{GroupDRO} aims to minimize the empirical worst-group loss formulated as:
% \begin{align}
%  \min_\theta \Big\{
%     \max_{g\in \mathcal{G}} \frac{1}{n_g} \sum_{i|g_i=g}^{n_g} \ell(f_\theta(x_i), y_i) \Big\}
% \end{align}
% where $n_g$ is the number of samples assigned to $g^\text{th}$ group.
% Unlike previous approaches, group DRO requires group annotations $g=(y,a)$ on the training split.
%%  Unlike Group DRO, we basically assume that we do not have group annotations in training data, and we are only given a small validation set with group annotations.
%
%\paragraph{Group reweighting (GR)}
% Using group annotations, we can extend class reweighting method to group reweighting one based on the inverse of group frequency in the training split, \ie,
%%  $\omega_i = n/{\sum_j \mathds{1}(y_j=y_i, a_j=a_i)}$.
%   \begin{align}
%    \min_\theta \Big\{\frac{1}{n}\sum_{i=1}^n \omega_i \ell(f_\theta(x_i), y_i) \Big\}~~\text{where}~~ \omega_i = \frac{n}{\sum_j \mathds{1}(y_j=y_i, a_j=a_i)}
%  \end{align}
% 
